An optimal transport problem with backward martingale constraints motivated by insider trading

We study a single-period optimal transport problem on $\mathbb{R}^2$ with a covariance-type cost function $c(x,y) = (x_1-y_1)(x_2-y_2)$ and a backward martingale constraint. We show that a transport plan $\gamma$ is optimal if and only if there is a maximal monotone set $G$ that supports the $x$-marginal of $\gamma$ and such that $c(x,y) = \min_{z\in G}c(z,y)$ for every $(x,y)$ in the support of $\gamma$. We obtain sharp regularity conditions for the uniqueness of an optimal plan and for its representation in terms of a map. Our study is motivated by a variant of the classical Kyle model of insider trading from Rochet and Vila (1994).

==> style.tex <==
% Packages

\usepackage{amsthm} \usepackage{amsmath} \usepackage{amsfonts}
\usepackage{amssymb} \usepackage{latexsym} \usepackage{enumerate}
\usepackage{mathrsfs}
\usepackage[round,authoryear]{natbib}
\usepackage[colorinlistoftodos, textwidth=4cm, shadow]{todonotes}
\usepackage{tikz}
\usepackage{pgfplots}

\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% Theorems and similar

\theoremstyle{plain}%
\newtheorem{Theorem}{Theorem}[section] %
\newtheorem{Corollary}[Theorem]{Corollary}%
\newtheorem{Lemma}[Theorem]{Lemma} %
\newtheorem{Proposition}[Theorem]{Proposition} %

\theoremstyle{definition}%
\newtheorem{Assumption}[Theorem]{Assumption}%
\newtheorem{Definition}[Theorem]{Definition}%
\newtheorem{Example}[Theorem]{Example} %
\newtheorem{Problem}[Theorem]{Problem} %
\newtheorem{Step}{Step}%
\theoremstyle{remark}%
\newtheorem{Remark}[Theorem]{Remark} %

% Useful commands

\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\braces}[1]{\left\lbrace{#1}\right\rbrace}
\newcommand{\descr}[2]{\left\lbrace{#1}:\; #2 \right\rbrace}
\newcommand{\diag}[1]{\mathrm{diag}(#1)}
\newcommand{\law}[1]{\Law(#1)}
% Various
\newcommand{\seq}[1]{$\left(#1^n\right)_{n\geq 1}$}
\newcommand{\set}{\triangleq}
\newcommand{\ip}[2]{\left\langle
    #1,#2 \right\rangle}
\newcommand{\pf}[2]{{#1}_{\#}{#2}}
\newcommand{\pr}[2]{\proj_{{#1}}({#2})}
\newcommand{\qv}[1]{\left\langle
    #1\right\rangle}
\newcommand{\idvec}{\mathbf{1}}
\newcommand{\mtext}[1]{\text{ #1 }}
\newcommand{\ind}[1]{1_{\braces{#1}}}
\newcommand{\setind}[1]{1_{#1}}
\newcommand{\cind}[1]{\delta_{#1}}
\newcommand{\map}[3]{#1:\; #2 \rightarrow #3} %1=name, 2=arg_domain, 3=val_domain
\newcommand{\norm}[1]{\lVert#1\rVert} %
\newcommand{\real}[1]{\mathbb{R}^{#1}}
\newcommand{\CM}{\textrm{(CM)}}
\newcommand{\sgn}{\operatorname{sgn}}

% Conditional expectation: measure, time, RV
\newcommand{\cE}[3]{\mathbb{E}\left(\left.#1\right\lvert\mathcal{F}^{#2}_{#3}\right)} 
\newcommand{\cEP}[2]{\mathbb{E}\left(\left.#1\right\lvert{#2}\right)}
\newcommand{\EP}[1]{\mathbb{E}\left(#1\right)}
\newcommand{\Prob}[2]{\mathbb{#1}\left(#2\right)} 
\newcommand{\PP}[1]{\Prob{\mathbb{P}}{#1}}

\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}


\newcommand{\cL}{\mathcal{L}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cP}{\mathcal{P}}

% Spaces
\newcommand{\sSpace}[2]{{{#1}_{#2}}}
\newcommand{\sNorm}[2]{\norm{#1}_{#2}}
\newcommand{\sH}[1]{{\sSpace{\mathcal{H}}{#1}}}
\newcommand{\sA}{\mathcal{A}}
\newcommand{\bmo}{\mathrm{BMO}}
\newcommand{\ms}[1]{\csupp{#1}}

% Operators

\newcommand{\Prj}[2]{\textrm{Pr}_{#2}(#1)}

% Mathematical operators

% \newcommand{\Arg}{\chi}

\DeclareMathOperator*{\argmax}{arg\:max}
\DeclareMathOperator*{\argmin}{arg\:min}
\DeclareMathOperator{\Arg}{Arg}
\DeclareMathOperator{\boundary}{\partial}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\closure}{cl}
\DeclareMathOperator{\cov}{Cov}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\udom}{\widehat{\dom}}
\DeclareMathOperator*{\esssup}{ess\:sup}
\DeclareMathOperator*{\essinf}{ess\:inf}
\DeclareMathOperator*{\interior}{int}
\DeclareMathOperator*{\ri}{ri}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\range}{range}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\csupp}{ms}
\DeclareMathOperator{\edom}{Dom_e}
\DeclareMathOperator{\graph}{graph}
\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\Law}{{Law}}
% Environments

\newcommand{\envspace}{\vspace{2mm}}
\newenvironment{ToDo}{\envspace
  \noindent {\textbf{Things to do:}}  \sf}{\envspace}
\newenvironment{ToThink}{\newline
  \noindent {\textbf{Note:}}  \sf}{\envspace}



